Towards a Scalable Dynamic Spatial Database System

With the rise of GPS-enabled smartphones and other similar mobile devices, massive amounts of location data are available. However, no scalable solutions for soft real-time spatial queries on large sets of moving objects have yet emerged. In this paper we explore and measure the limits of actual algorithms and implementations regarding different application scenarios. And finally we propose a novel distributed architecture to solve the scalability issues.

==> summarytable.tex <==

\begin{table}[ht]
\centering
\label{tab:summarytable}
\begin{tabular}{ r | c || c | c }
  scenario     & T   & CGAL & PostGIS \\
  \hline\hline\noalign{\smallskip}
          car fleet	&  1min &   650K	&   20K \\
          	 		&  10s  &   40K    &   3000 \\
\hline\noalign{\smallskip}
        battlefield	&  1sec  &   18K	&   300 \\
 		awareness	&  10ms  &   100	&   - \\
%\hline\noalign{\smallskip}
%      pervasive 	&  10min  &   5M 	&   200K\\
%        robotics	&  10s    &   65K 	&   3000\\
\hline\noalign{\smallskip}
              local &  10min  &  5M	&   200K \\
  		advertising	&  20s  &  120K	&   6000 \\
\hline\noalign{\smallskip}
             social &  30min  &  70M 	&   600K\\
			network	&  20s  &  160K 	&   6000\\
\hline\noalign{\smallskip}
             hybrid &  100ms  & 1000	&   30 \\
     	 reality	&  30ms  & 300	&   10 \\
\end{tabular}
%\captionsetup{labelformat=empty,justification=centering}
\caption{Maximum number of moving objects using CGAL or PostGIS for each application scenario\\T is the mean time between two position updates}
\end{table}


